CaesarNeRF: Calibrated Semantic Representation for Few-shot Generalizable Neural Rendering

Generalizability and few-shot learning are key challenges in Neural Radiance Fields (NeRF), often due to the lack of a holistic understanding in pixel-level rendering. We introduce CaesarNeRF, an end-to-end approach that leverages scene-level CAlibratEd SemAntic Representation along with pixel-level representations to advance few-shot, generalizable neural rendering, facilitating a holistic understanding without compromising high-quality details. CaesarNeRF explicitly models pose differences of reference views to combine scene-level semantic representations, providing a calibrated holistic understanding. This calibration process aligns various viewpoints with precise location and is further enhanced by sequential refinement to capture varying details. Extensive experiments on public datasets, including LLFF, Shiny, mip-NeRF 360, and MVImgNet, show that CaesarNeRF delivers state-of-the-art performance across varying numbers of reference views, proving effective even with a single reference image.

==> tables/ablation_perceptual.tex <==

\begin{table}[tb]
\centering
\def\lw{1.3}
\def\lk{2.4}
\def\ls{0.06}
%\scriptsize
\resizebox{.9\linewidth}{!}
{
\begin{tabular}{p{1.9cm}p{\ls cm}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}} \toprule

\multirow{1}{*}{Perceptual} && PSNR  & LPIPS & SSIM  \\
\midrule
 GNT && 20.93 & 0.185 & 0.731 \\
 \midrule

\bottomrule
\end{tabular}
}
\medskip
\caption{Ablation results on type and weight of perceptual loss.} 
\label{tab:perc_ablation}
\end{table}

==> tables/main_full_generalizable.tex <==

\begin{table}[tb]
\centering
\def\lw{1.5}
\def\lk{2.4}
\def\ls{0.0}
%\scriptsize
\resizebox{.9\linewidth}{!}
{
\begin{tabular}{p{2.5cm}p{\ls cm}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}} \toprule

\multirow{1}{*}{Method} && PSNR ($\uparrow$) & LPIPS ($\downarrow$) & SSIM ($\uparrow$)  \\
\midrule
PixelNeRF \cite{yu2021pixelnerf}    && 18.66 & 0.463 & 0.588  \\
MVSNeRF \cite{chen2021mvsnerf}      && 21.18 & 0.301 & 0.691  \\
IBRNet \cite{wang2021ibrnet}        && 25.17 & 0.200 & 0.813  \\
NeuRay \cite{liu2022neural}         && 25.35 & 0.198 & 0.818  \\
GeoNeRF \cite{johari2022geonerf}    && \cellcolor{yellow!40}25.44 & 0.180 & 0.839  \\
ContraNeRF \cite{yang2023contranerf} && \cellcolor{yellow!40}25.44 & 0.178 & 0.842 \\
GPNR \cite{suhail2022generalizable} && \cellcolor{red!40}25.72 & \cellcolor{yellow!40}0.175 & \cellcolor{red!40}0.880  \\
GNT \cite{varma2022attention}       && \cellcolor{orange!40}25.65 & \cellcolor{orange!40}0.140 & \cellcolor{orange!40}0.853  \\
Ours                                && 25.17 & \cellcolor{red!40}0.137 & \cellcolor{yellow!40}0.852  \\
 \midrule
\end{tabular}
}
\medskip
\caption{Generalizable results on LLFF \cite{mildenhall2019local} compared with state-of-the-art methods using all reference views as input.} 
\label{tab:main_generalizable}
\end{table}

==> tables/main_per_scene.tex <==

\begin{table*}[tb]
\centering
\caption{Full table of evaluation for per-scene optimization of eight categories on the LLFF~\cite{mildenhall2019local} dataset comparing CaesarNeRF with state-of-the-art methods. } 
\label{tab:main_llff_per_scene}
\def\lw{1.5}
\def\ls{0.06}
%\scriptsize
\resizebox{\linewidth}{!}
{
\begin{tabular}{p{1.5cm}p{1.9cm}p{\ls cm}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}p{\lw cm}<{\centering}} \toprule
%\multirow{2}{*}{Input}& \multirow{2}{*}{Method} &&\multicolumn{3}{c}{Real Forward-Facing} && \multicolumn{3}{c}{Blender} && \multicolumn{3}{c}{MVImgNet} \\
\multirow{1}{*}{Metric}& \multirow{1}{*}{Method} && trex & fern & flower & leaves & room & fortress & horns & orchids\\%{MVImgNet} \\
\midrule
%\cline{1-2} \cline{4-11} \\ [-8pt]
\multirow{5}{*}{PSNR ($\uparrow$)} 
& LLFF \cite{mildenhall2019local} && 27.48 & \cellcolor{gray!50}28.72 & 20.72 & 21.13 & 24.54 & 21.79 & 23.22 & 18.52\\
& NeRF \cite{mildenhall2021nerf}  && 26.80 & 25.17 & 27.40 & 20.92 & 32.70 & 31.16 & 27.45 & 20.36\\
& NeX \cite{wizadwongsa2021nex} && \cellcolor{gray!50}28.73 & 25.63 & \cellcolor{gray!50}28.90 & 21.96 & 32.32 & 31.67 & 28.46 & 20.42\\
%& NLF \cite{suhail2022light} && 30.34 & 24.86 & 29.82 & 22.47 & 34.53 & 33.22 & 29.78 & 21.05\\
& GNT \cite{varma2022attention}   && 28.15 & 24.31 & 27.32 & 22.57 & \cellcolor{gray!50}32.96 & 32.28 & \cellcolor{gray!50}29.62 & 20.67\\
& Ours                            && 28.30 & 25.63 & 28.29 & \cellcolor{gray!50}23.11 & 32.21 & \cellcolor{gray!50}32.47 & 29.56 & \cellcolor{gray!50}21.52\\
\midrule
\multirow{5}{*}{LPIPS ($\downarrow$)}
& LLFF \cite{mildenhall2019local} && 0.222 & 0.247 & 0.174 & 0.216 & 0.155 & 0.173 & 0.193 & 0.313\\
& NeRF \cite{mildenhall2021nerf}  && 0.249 & 0.280 & 0.219 & 0.316 & 0.178 & 0.171 & 0.263 & 0.321\\
& NeX \cite{wizadwongsa2021nex} && 0.193 & 0.205 & 0.150 & 0.173 & 0.161 & 0.131 & 0.173 & 0.242\\
%& NLF \cite{suhail2022light} && 0.143 & 0.135 & 0.107 & 0.110 & 0.104 & 0.119 & 0.121 & 0.173\\
& GNT \cite{varma2022attention}   && 0.080 & 0.116 & 0.092 & 0.109 & 0.060 & 0.061 & 0.076 & 0.153\\
& Ours                            && \cellcolor{gray!50}0.076 & \cellcolor{gray!50}0.111 & \cellcolor{gray!50}0.068 & \cellcolor{gray!50}0.095 & \cellcolor{gray!50}0.057 & \cellcolor{gray!50}0.055 & \cellcolor{gray!50}0.071 & \cellcolor{gray!50}0.139\\
\midrule
\multirow{5}{*}{SSIM ($\uparrow$)}
& LLFF \cite{mildenhall2019local}   && 0.857 & 0.753 & 0.844 & 0.697 & 0.932 & 0.872 & 0.840 & 0.588\\
& NeRF \cite{mildenhall2021nerf}    && 0.880 & 0.792 & 0.827 & 0.690 & 0.948 & 0.881 & 0.828 & 0.641\\
& NeX \cite{wizadwongsa2021nex}  && \cellcolor{gray!50}0.953 & \cellcolor{gray!50}0.887 & \cellcolor{gray!50}0.933 & 0.832 & \cellcolor{gray!50}0.975 & \cellcolor{gray!50}0.952 & 0.937 & 0.765\\
%& NLF \cite{suhail2022light} && 0.963 & 0.886 & 0.939 & 0.856 & 0.987 & 0.964 & 0.957 & 0.807\\
& GNT \cite{varma2022attention}     && 0.936 & 0.846 & 0.893 & 0.852 & 0.963 & 0.934 & 0.935 & 0.752\\
& Ours                              && 0.943 & 0.871 & 0.912 & \cellcolor{gray!50}0.872 & 0.967 & 0.946 & \cellcolor{gray!50}0.939 & \cellcolor{gray!50}0.782\\
\bottomrule
\end{tabular}
}
\end{table*}
